Data-Aware Gradient Compression for FL in Communication-Constrained Mobile Computing

Federated Learning (FL) in mobile environments faces significant communication bottlenecks. Gradient compression has proven as an effective solution to this issue, offering substantial benefits in environments with limited bandwidth and metered data. Yet, it encounters severe performance drops in non-IID environments due to a one-size-fits-all compression approach, which does not account for the varying data volumes across workers. Assigning varying compression ratios to workers with distinct data distributions and volumes is therefore a promising solution. This work derives the convergence rate of distributed SGD with non-uniform compression, which reveals the intricate relationship between model convergence and the compression ratios applied to individual workers. Accordingly, we frame the relative compression ratio assignment as an $n$-variable chi-squared nonlinear optimization problem, constrained by a limited communication budget. We propose DAGC-R, which assigns conservative compression to workers handling larger data volumes. Recognizing the computational limitations of mobile devices, we propose the DAGC-A, which is computationally less demanding and enhances the robustness of compression in non-IID scenarios. Our experiments confirm that the DAGC-R and DAGC-A can speed up the training speed by up to $25.43\%$ and $16.65\%$ compared to the uniform compression respectively, when dealing with highly imbalanced data volume distribution and restricted communication.

==> sections/Bio.tex <==
\section*{Biography Section} \label{Bio}
\vspace{-2cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Bio/rongweiLu.jpg}}]{Rongwei Lu}
is currently a Ph.D. student in Computer Technology at Tsinghua University. His research interests include distributed machine learning, federated learning and large scale machine learning systems. He was a research intern in the System Research Group of MSRA in 2023. He has published papers in conferences such as IEEE INFOCOM. He has served as a reviewer for NeurIPS, MM and ICLR.
\end{IEEEbiography}
\vspace{-2cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Bio/yutongJiang.jpg}}]{Yutong Jiang}
is currently pursuing the Master's degree in Computer Technology at Tsinghua University. Her research interests focus on optimization and acceleration of distributed machine learning.
\end{IEEEbiography}
\vspace{-2cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Bio/yinanMao.jpg}}]{Yinan Mao}
is currently an algorithm engineer in the AI cloud business group of Baidu Incorporated. He received his Master’s degree in Computer Technology from Tsinghua University. His research interests are to optimize accuracy of peer content delivery networks using meta-learning and sampling strategy. He was a research intern in the Industry Robot Group of ByteDance in 2022 and 2023. He has published several papers in conferences and journals such as IEEE IGARSS, ICME and TMM.
\end{IEEEbiography} 

\vspace{-1cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Bio/chenTang.jpg}}]{Chen Tang }
is currently a research assistant in the Department of Computer Science and Technology at Tsinghua University. He received his Master's degree in Computer Technology from Tsinghua University. He was a research intern in System and Networking Research Group of Microsoft Research Asia (MSRA) and was a visiting student of Peng Cheng National Laboratory (PCL). 
He has published several papers on top-tier conferences, including ACM MM, ECCV, ICCV, and EMNLP. 
He has served as a reviewer for CVPR, ECCV, ECAI, ICLR, and NeurIPS. 
His research interests are in efficient deep learning (e.g., quantization, sparsity), hardware-aware neural architecture search, and dynamic neural networks. 
\end{IEEEbiography} 

\vspace{-1cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Bio/binChen.jpg}}]{Bin Chen }
received the B.S. and M.S. degrees in mathematics from South China Normal University, Guangzhou, China, in 2014 and 2017, respectively, and Ph.D. degree from the Department of Computer Science and Technology, Tsinghua University, Beijing, China, in 2021. From December 2019 to May 2020, he visited Department of Electrical and Computer Engineering, University of Waterloo, Canada. From May 2021 to November 2021, he was a Post-Doctoral Researcher with the Shenzhen International Graduate School, Tsinghua University, Shenzhen. Since December 2021, he has been an Associate Professor with the Department of Computer Science and Technology, Harbin Institute of Technology, Shenzhen, China. His research interests include Coding and Information Theory, Multimedia Compression, and AI Security.
\end{IEEEbiography}

\vspace{-1cm}

 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Bio/laizhongCui.jpg}}]{Laizhong Cui}
is currently a Professor in the College of Computer Science and Software Engineering at Shenzhen University, China. He received the B.S. degree from Jilin University, Changchun, China, in 2007 and Ph.D. degree in computer science and technology from Tsinghua University, Beijing, China, in 2012. His research interests include Future Internet Architecture and Protocols, Edge Computing, Multimedia Systems and Applications, Blockchain, Internet of Things, Cloud Computing and Federated Learning. He led more than 10 scientific research projects, including National Key Research and Development Plan of China, National Natural Science Foundation of China, Guangdong Natural Science Foundation of China and Shenzhen Basic Research Plan. He has published more than 100 papers, including IEEE JSAC, IEEE TC, IEEE TPDS, IEEE TKDE, IEEE TMM, IEEE TMC, IEEE IoT Journal, IEEE TII, IEEE TNSM, ACM TOIT, IEEE Network, IEEE INFOCOM, ACM MM, IEEE ICNP, IEEE ICDCS, etc. He serves as an Associate Editor or a Member of Editorial Board for several international journals, including IEEE Internet of Things Journal, IEEE Transactions on Cloud Computing, IEEE Transactions on Network and Service Management, and International Journal of Machine Learning and Cybernetics. He is a Senior Member of the IEEE, and a Distinguished Member of the CCF.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Bio/zhiWang.png}}]{Zhi Wang}
is currently an associate professor at Shenzhen International Graduate School, Tsinghua University. 
He received his Ph.D. in 2014 and his B.E. in 2008, both from Department of Computer Science and Technology, Tsinghua University. 
His research areas include multimedia networks, mobile cloud computing, and large-scale machine learning systems. 
He is a recipient of the Natural Science Award of the Ministry of Education (First Prize) in 2017, 
the National Natural Science Award (Second Prize) in 2018, the Shenzhen Youth Science and Technology Award in 2019, 
and the Technology Invention Award of the Chinese Institute of Electronics (First Prize) in 2020. 
In addition, his research won the Best Paper Award of ACM Multimedia, Best Paper Award of IEEE TMM, 
the Outstanding Doctoral Thesis Award of China Computer Federation, the Best Student Paper Award of MMM, 
and the Best Paper Award of ACM Multimedia, HUMA Workshop. He is an Associate Editor of IEEE TMM and Guest Editor of ACM TIST and JCST. 
His research has been covered by prestigious technology media, including MIT Technology Review and Synced Review.
\end{IEEEbiography}
